The Use of Instrumentation in Grammar Engineering

This paper explores the usefulness of a technique from software engineering, code instrumentation, for the development of large-scale natural language grammars. Information about the usage of grammar rules in test and corpus sentences is used to improve grammar and testsuite, as well as adapting a grammar to a specific genre. Results show that less than half of a large-coverage grammar for German is actually tested by two large testsuites, and that 10--30% of testing time is redundant. This methodology applied can be seen as a re-use of grammar writing knowledge for testsuite compilation.

==> nobi-hyphen.tex <==
\hyphenation{
Adjektiv-endun-gen
Allo-morph-re-geln
Allo-morphe
Allo-morphie
Ana-lyse-pro-gramm
Analyse-protokoll
De-fini-tion
Dis-kurs-wissen
Hash-funk-tio-nen
Hash-funk-tion
Haupt-speicher
Im-ple-men-tation
Kate-gorien
Kla-ssi-fi-ka-tion
Kombi-nations-regeln
Lama
Lexikon-organi-sation
Nomina
Para-digma
Parti-zipI
%Pr"afixe
Pro-gramm
Sprach-ana-lyse-sys-tem
Sys-tems
TRUE
Teil-auf-gabe
Unifikations-formalis-mus
Verb-le-xi-kon
Verb-le-xi-kons
Wort-analysen
Wort-seman-tik
an-dere
aus-gehend
be-deutungs-tragende
be-nutzt
beruf-liche
buch-staben-orien-tiert
buch-staben-orien-tierten
dies
ka-te-go-ri-siert
morphem-orientiert
regexp
%re-pr"asentiert
spe-zielle
}

